DeepLENS: Deep Learning for Entity Summarization

Entity summarization has been a prominent task over knowledge graphs. While existing methods are mainly unsupervised, we present DeepLENS, a simple yet effective deep learning model where we exploit textual semantics for encoding triples and we score each candidate triple based on its interdependence on other triples. DeepLENS significantly outperformed existing methods on a public benchmark.

==> 4-relatedwork.tex <==
\section{Related Work}\label{sec:relatedwork}

Existing methods for entity summarization are mainly unsupervised. To assess the informativeness of a triple, RELIN~\cite{relin} relies on information theory, while KAFCA~\cite{kafca} uses the depths of triples in a hierarchy constructed by Formal Concept Analysis. BAFREC~\cite{bafrec} only uses depths for meta-level triples, but calculates frequencies for data-level triples. LinkSUM~\cite{linksum} computes PageRank and exploits backlinks. To improve the diversity of a summary, DIVERSUM~\cite{diversum} chooses triples having different properties. FACES~\cite{faces} and FACES-E~\cite{facese} cluster triples and choose top-ranked triples from as many clusters as possible. CD~\cite{cd} formulates a quadratic knapsack problem to minimize the similarity between selected triples. MPSUM~\cite{mpsum} constructs a Latent Dirichlet Allocation model for ranking triples, where each property as a topic is a distribution over values.

To the best of our knowledge, ESA~\cite{esa} is the only supervised method for general-purpose entity summarization. ESA encodes RDF resources using both word embedding and graph embedding, whereas we only rely on word embedding. ESA encodes a set of triples as a sequence fed into BiLSTM, whereas our aggregation-based representation is permutation invariant.
